Spot Transit: Cheaper Internet Transit for Elastic Traffic

We advocate to create a \emph{spot} Internet transit market, where transit is sold using the under-utilized backbone capacity at a lower price. The providers can improve profit by capitalizing the perishable capacity, and customers can buy transit on-demand without a minimum commitment level for elastic traffic, and as a result improve its surplus (i.e. utility gains). We conduct a systematic study of the economical benefits of spot transit both theoretically and empirically. We propose a simple analytical framework with a general demand function, and solve the pricing problem of maximizing the expected profit, taking into account the revenue loss of regular transit when spot transit traffic hikes. We rigorously prove the price advantage of spot transit, as well as profit and surplus improvements for tier-1 ISPs and customers, respectively. Using real-world price data and traffic statistics of 6 IXPs with more than 1000 ISPs, we quantitatively evaluate spot transit and show that significant financial benefits can be achieved in both absolute and relative terms, robust to parameter values.

==> dynamic.tex <==
\section{Dynamic Pricing for Revenue Maximization}
\label{sec:dynamic}

We have studied the optimal static pricing policy to maximize expected revenue amid uncertain demand in Sec.~\ref{sec:static}. Instead of relying on a static price, the ISP can adopt a \emph{dynamic pricing} policy that adjusts the price to react to the demand changes on the spot and has the potential to further improve the revenue. The scenario is similar to cloud computing companies, such as Amazon, selling the so-called ``spot instances'' whose price varies according to the supply and demand relationship dynamically \cite{amazonspot}. In this section, we study the dynamic pricing problem by formulating and solving it as an average reward dynamic program.

Instead of focusing on the aggregated quantity of demand as in the preceding analysis, we need to consider individual demand arrivals and departures and instantaneous bandwidth utilization when dealing with dynamic pricing. The basic intuition is that, whenever the bandwidth utilization is high and demand arrivals are frequent, the price has to be increased to prevent demand overflow from happening, and to obtain more revenue from current users. On the other hand, if the bandwidth utilization is low, the price then has to be decreased to offer a discounted service to stimulate demand and improve revenue potential in the long run. The ISP's objective is the average expected revenue. Thus, we must consider the effects of pricing on both the present revenue and the future potential. This is naturally a dynamic program.

\subsection{Model}
\label{subsec:dynamic_model}

Since now we have to focus on individual demand arrival and departure, we no longer have demand as a random variable but instead as a \emph{random process}. Particularly, we assume that demand is affected by two independent stochastic processes, namely the arrival process that corresponds to the birth of new traffic, and the departure process that models the death of existing demand (when traffic disappears). At price $p$, demand arrival can be expressed as a Poisson process with a rate $\lambda(p)$ (volume of new traffic per time unit). Intuitively, as price $p$ increases, customers have less financial incentive to use the service, therefore a lower arrival rate.

We also assume the existence of a \emph{null price} $p^{\max}$ for $\lambda(p)$, at which the arrival rate equals $0$. Mathematically, this is used to model the demand overflow scenario as an implicit constraint that forces the ISP to price at $p^{\max}$ when spot capacity is fully utilized, i.e. $n=C$. This ensures that demand overflow will not happen with dynamic pricing, and is commonly used on economics literature \cite{EK03}.

The demand departure process is also modeled as a Poisson process with rate $\theta(p)$, where $\theta$ is the departure rate function. When $p$ decreases, customers naturally have a lower probability to leave the system, resulting in a lower departure rate. $\lambda$ and $\theta$ can be estimated from past demand data, and this process can be refined periodically. 

The price is a function of system state. The cardinality of the state space $\mathcal{K}$ has to be finite for the problem to be tractable, where $\mathcal{K}$ represents all possible spot bandwidth utilization up to the capacity $C$. Thus we must discretize utilization. We assume that the ISP chooses a value for the discretization step $\Delta C=1$ Gbps, and the cardinality of the state space is $K=|\mathcal{K}|=C$. The ISP charges $p_n$ if the instantaneous spot bandwidth usage is in state $n$, i.e. the system utilization falls within $[n-1, n]$ Gbps. Finer state space discretization means that pricing would change with a small change in utilization, and is therefore more dynamic.


\subsection{Formulation}

The revenue maximization problem can be formulated as follows. The goal of the ISP is to maximize the average revenue in the infinite horizon. This quantity is denoted by $J$. A pricing policy is a rule that determines which price should be advertised at any given time as a function of the current state $n$. We are interested in finding a pricing policy $\pmb{p}=\{ p_1,p_2,\ldots,p_K \}$ that achieves this goal, from the set $\mathcal{P}=\{ \pmb{p} | 0\le p_n \le p^{\max},\forall n \}$ of all possible pricing policies.

Under the assumptions in Sec.~\ref{subsec:dynamic_model}, the system follows the dynamics of a continuous-time birth-death Markov process, and explicit expression for the average profit $J$ can be provided as follows. First, we denote the steady-state probability of state $n$ given a pricing policy $\pmb{p}$ as $\pi_n(\pmb{p})$. The arrival and departure rates in any state given $\pmb{p}$ can be readily obtained, and the steady-state probabilities $\pi_n(\pmb{p})$ is as follows:
\begin{equation*}
    \pi_n(\pmb{p})=\frac{\frac{\lambda_0 \lambda_1 \lambda_2 \ldots \lambda_{n-1}}{\theta_1\theta_2\ldots\theta_n}}{1+\frac{\lambda_0}{\theta_1}+\frac{\lambda_0\lambda_1}{\theta_1\theta_2}+\ldots+\frac{\lambda_0 \lambda_1 \lambda_2 \ldots \lambda_{K-1}}{\theta_1\theta_2\ldots\theta_K}}
\end{equation*}

Due to the Poisson Arrivals See Time Averages property, the average revenue is
\begin{equation*}
  J(\pmb{p}) = \sum^C_{n=0} \pi_n (\pmb{p})\cdot n p_n,
\end{equation*}
since price is charged on a usage basis for transit bandwidth.

The provider's problem is to find a pricing policy $\pmb{p^*}$ that maximizes the average revenue denoted by $J^*$. Equivalently,
\begin{equation}\label{eqn:opt}
  J^* \doteq \sup_{\pmb{p}\in\mathcal{P}} J(\pmb{p}).
\end{equation}
This is a finite-state, continuous-time, average reward dynamic programming problem. Note that the set $\mathcal{P}$ is compact and all states communicate, so there always exists a policy with which we can eventually reach an arbitrary state $n'$ from any state $n$. The demand arrival and departure functions $\lambda(p)$ and $\theta(p)$ are all continuous, and thus the transition rates and the average reward $J$ are continuous in the decision variables $p_n$s. Moreover, the reward and the expected holding time at each state $n$, and the total transition rate out of any state are all bounded functions of $\pmb{p}$. Under these conditions, the standard DP theory applies \cite{B76}, and there exists a stationary policy which is optimal.

\subsection{Optimality Conditions}

\eqref{eqn:opt} is a complex stochastic dynamic program. To solve it, we can consider the so-called Bellman's equations since all the states in the Markov chain are recurrent. Bellman's equations are formulated for discrete-time Markov chains. Thus, we need to discretize our Markov chain by a procedure called \emph{uniformization}, where the transition rates out of each state are normalized by the maximum possible transition rate $v$, which in our case is given by 
\begin{equation}\label{eqn:v}
  v = \max_p\ \lambda(p) + \theta(p).
\end{equation}
The uniformized Markov chain for our problem is illustrated in Fig.~\ref{fig:markov}.
\begin{figure}[htp]
\centering
\includegraphics[width=0.48\textwidth]{figures/markov}
\vspace{-2mm}
\caption{The uniformized Markov chain for our problem.}
\label{fig:markov}\vspace{-2mm}
\end{figure}

With the above setup, we can obtain the Bellman's equations of the following form:
\begin{multline}\label{eqn:opt_cond_dp}
  J^* + h_n = \max_{{p_n}\in \mathcal{P}} \bigg[ np_n
  +  \frac{\lambda(p_n)}{v} h_{n+1} + \frac{\theta(p_n)}{v} h_{n-1} \\
  +  \left(1-\frac{\lambda(p_n)}{v}-\frac{\theta(p_n)}{v}\right) h_n \bigg],
\end{multline}
for $n = 1, 2, \ldots, K-1$. The first term in the right hand side is the revenue in state $n$. The second, third, and fourth terms are contributions to the revenue if the next transition is a demand arrival, a departure, or a recurrence, respectively. The unknowns in the above equations are $h_n$ and $J^*$. $J^*$ represents the optimal expected revenue as discussed, and $h_n$ denotes the \emph{relative reward} in state $n$. In particular, consider an optimal pricing policy that attains the maximum in \eqref{eqn:opt_cond_dp} for every state $n$. If we follow this policy starting from state $n'$ or state $n$, the expectation of the difference in total revenue gained over the \emph{infinite} horizon is equal to $(h_{n'}-h_n)/v$.

Note that \eqref{eqn:opt_cond_dp} holds only for $n\in [1,K-1]$. To deal with cases when $n=0$ and $K$, i.e. when there is no demand departure and arrival, respectively, we can simply let $h_{-1} = 0$, and $h_{K+1}=h_{K}$.

The solution to the Bellman's equations can be computed using classical DP algorithms such as the policy iterations or relative value iteration \cite{B76}. The resulted prices that maximize the right-hand side of \eqref{eqn:opt_cond_dp} at each state $n$ constitutes the optimal pricing policy $\pmb{p}^*$. %However, the computational complexity increases with the size of the state space $C$, which is generally large for a large-scale datacenter. For this reason, numerically computing an exact solution using DP can be 


\subsection{Structural Results}
\label{subsec:thm}
Although we have found the Bellman's equations, obtaining a closed form solution is quite difficult for arbitrary demand arrival and departure functions. Numerical algorithms also suffer from the so-called ``curse of dimensionality'' for large-scale problems. We are able to characterize several important structural properties of the optimal solution to the dynamic program \eqref{eqn:opt_cond_dp}, which can be used for designing simpler yet effective heuristics. 

Our first result is the monotonicity of the relative rewards. It corresponds to the fact that it is more desirable to have a higher utilization of the spot capacity, as they lead to higher revenue in the long run even though they imply fewer revenue opportunities in the future.
\begin{theorem}\label{thm:h}
  \textbf{Monotonicity of $h_n$.} $h_{n+1}\ge h_{n}$ for all $n=0,1,\ldots,K-1$. 
\end{theorem}
\begin{proof}
    Fix some $n, n\in[0,K-1]$. Now consider two copies of the system. System A starts from state $n$ and follows the optimal pricing policy $\pmb{p^*}$. System B starts with $n+1$, and uses the same price at any point of time as System A. Therefore the statistics of the arrival processes for the two systems are identical, and by defining the two processes on a common probability space, we can assume that the actual arrivals are the same. We can also identify the common $n$ of the customers in System B with those in System A so that they have identical departure times. Thus, at any give time, the state of System A is always less than that of System B, and so is the revenue since prices are identical. That is, $h'(n+1)>h_n$, where $h'(n+1)$ denotes the relative reward starting from state $n+1$ with this particular pricing policy. By definition, we have $h_{n+1}>h'(n+1)$. Thus we conclude that $h_{n+1}>h_n$.
\end{proof}

We can further show that the relative rewards exhibit diminishing marginal returns with respect to utilization.
\begin{theorem}\label{thm:h_concavity} 
  \textbf{Concavity of $h_n$.} $h_n$ is concave in $n$ for all $n=1,2,\ldots,K-1$.
\end{theorem}
\begin{proof}
  It suffices to show that
  \begin{equation}
    h_n - h_{n-1} \ge h_{n+1} + h_n, \forall n\in[1,K-1].
  \end{equation}
  The proof follow similar methods to those used in \cite{PT00}. The difference lies in taking into consideration the usage based charging instead of a fixed rate charging in \cite{PT00}. It is omitted here due to space constraints.
  %We prove by constructing a feasible pricing policy that satisfies the above inequality at equality.

  %Consider three copies of the system, System A, B, and C, respectively. System A starts from state $n-1$ and follows the optimal policy. System B starts from state $n+1$ and also follows the optimal policy.  The third copy of the system, System C, starts from state $n$, and at any point in time, it sets the price as half of the sum of System A's and B's prices. Let $h'_n$ denote the relative reward obtained from this particular pricing policy. Now by construction of the policy and the definition of $h_n$, we have
%\begin{equation*}
  %h'_n = \frac{1}{2}(h_{n-1}+h_{n+1}).
%\end{equation*}
  %Since $h_n$ corresponds to the relative reward obtained from the optimal policy, $h_n \ge h'_n$, and thus the proof.  
\end{proof}

%This concavity property of the optimal revenue is not only crucial for further development of this paper, but also of interest in itself. For example, it can be useful for determining the optimal number of instances running in the system if it is part of the decisions. When the cost of providing computing hardware is linear or strictly convex, the expected profit becomes a concave function of the number of running instances. In this case, the optimal utilization is the largest quantity for which the marginal expected revenue exceeds the marginal cost.

We can now prove our main result, i.e. the monotonicity of the optimal price at each state.

\begin{theorem}\label{thm:p}
  \textbf{Price Monotonicity.} $p^*_{n} \ge p^*_{n-1}$ for $n=1,2,\ldots,K$.
\end{theorem}

\begin{figure*}[ht]
\centering\vspace{-2mm}
\subfigure[Optimal price.]{
\includegraphics[width=0.48\linewidth]{figures/price1-3}
\label{fig:price123}
}
\subfigure[Expected revenue difference $h_n/v$.]{
\includegraphics[width=0.48\linewidth]{figures/reward1-3}
\label{fig:reward123}
}
\subfigure[Optimal price.]{
\includegraphics[width=0.48\linewidth]{figures/price514}
\label{fig:price514}
}
\subfigure[Expected revenue difference ${h_n}/{v}$.]{
\includegraphics[width=0.48\linewidth]{figures/reward514}
\label{fig:reward514}
}
\vspace{-2mm}
\caption[]{Numerical results with $K=100$, $|\mathcal{P}|=1000$, $\lambda(p)=24-1.5p^2$, and $p^{\max}=4$.}
\label{fig:results_dp}
\vspace{-4mm}
\end{figure*}

\begin{proof}
  For convenience, let us denote $j_n=h_{n+1} - h_n$. From Theorem~\ref{thm:h_concavity} we know that $j_n\le j_{n-1}$. Re-arranging the terms in \eqref{eqn:opt_cond_dp} we have
\begin{gather}\label{eqn:g}
   J^* = n p^*_n + j_n \frac{\lambda(p^*_n)}{v} - j_{n-1}\frac{\theta(p^*_{n})}{v}.
\end{gather}
By the definition of the optimal price $p^*_n$ for state $n$, any other price cannot make the right-hand side of \eqref{eqn:g} larger, i.e.
\begin{gather*}
  J^* \ge n p^*_{n-1} + j_n \frac{\lambda(p^*_{n-1})}{v} - j_{n-1}\frac{\theta(p^*_{n-1})}{v},
\end{gather*}
which gives us
\begin{gather*}
  p^*_n - p^*_{n-1} \ge \\
  \frac{1}{nv}\bigg[ j_n \big(\lambda(p^*_{n-1}) - \lambda(p^*_n)  \big) + j_{n-1} \big( \mu(p^*_n) - \theta(p^*_{n-1}) \big) \bigg]
\end{gather*}
Similarly we can write
\begin{gather*}
  J^* = (n-1) p^*_{n-1} + j_{n-1} \frac{\lambda(p^*_{n-1})}{v} - j_{n-2}\frac{\theta(p^*_{n-1})}{v}\\
  \ge (n-1) p^*_{n} + j_{n-1} \frac{\lambda(p^*_{n})}{v} - j_{n-2}\frac{\theta(p^*_{n})}{v}\\
  \hspace{-60mm} \Rightarrow p^*_n - p^*_{n-1} \le \\
  \frac{1}{(n-1)v}\bigg[ j_{n-1} \big(\lambda(p^*_{n-1}) - \lambda(p^*_n) \big) + j_{n-2} \big( \theta(p^*_n) - \theta(p^*_{n-1}) \big) \bigg]
\end{gather*}

Thus for the two inequalities to hold, we must have
\begin{gather*}
  \frac{1}{nv}\bigg[ j_n \big(\lambda(p^*_{n-1}) - \lambda(p^*_n)  \big) + j_{n-1} \big( \theta(p^*_n) - \theta(p^*_{n-1}) \big) \bigg] \le \\
  \frac{1}{(n-1)v}\bigg[ j_{n-1} \big(\lambda(p^*_{n-1}) - \lambda(p^*_n) \big) + j_{n-2} \big( \theta(p^*_n) - \theta(p^*_{n-1}) \big) \bigg],
\end{gather*}
which holds only when $p^*_{n} \ge p^*_{n-1}$ since $\lambda'(p) < 0, \theta'(p)>0$, and $0\le j_n \le j_{n-1} \le j_{n-2}$.
\end{proof}

Theorem~\ref{thm:p} has natural economic interpretations. When the system is heavily loaded, it is in the interest of the ISP to set a higher price to obtain higher revenue, as well as to discourage future demand in order to prevent the system from demand overflow. When the system is lightly utilized, the provider can afford to adopt a lower price to attract more customers. 


\subsection{Numerical Studies}
\label{subsec:dynamic_evaluation}

In this section, we conduct numerical studies to evaluate the properties of the optimal dynamic pricing policy. Recall that the unit of bandwidth is Gbps, and the unit of price is \$K/Gbps. We let $K=C=100$, which means that the capacity is $100$ Gbps and the state space is discretized into $100$ states. The ISP thus considers a dynamic pricing policy with $100$ price points. The action space $\mathcal{P}$ that contains all possible prices is also discretized. We set the cardinality of the action space to be $1000$, which means that each of the $100$ price points is chosen from a total of $1000$ possible values. Note that finer granularity discretization leads to better numerical results, but also incurs higher computational burden. 

We use the arrival rate function $\lambda(p)=24-1.5p^2$ throughout the simulations, with different departure rate functions $\theta(p)$ to demonstrate the effect of demand dynamics on pricing and revenue. $p^{\max}=4$ in this case. We solve the dynamic program with the Matlab Markov Decision Processes Toolbox developed by INRA \cite{mdptoolbox}. Both policy iteration and relative value iteration can be used. Policy iteration theoretically requires on the order of $O(|\mathcal{P}|^K)$ iterations to converge while value iteration is not guaranteed to converge within a finite number of steps. However value iteration has a lower computational complexity at each iteration. In practice, policy iteration appears to converge faster \cite{BT00} and is used to solve our problem with the boundary condition $h_K=0$. 

Fig.~\ref{fig:price123} and Fig.~\ref{fig:reward123} show the optimal prices and expected revenue differences ($h_n/v$) with a class of departure rate functions $\theta(p)=cp^2$, where $c=0.3$, $1.5$, and $3$, respectively. First, notice that $p^*_n$ increases with $n$ as predicted in Theorem~\ref{thm:p}. When $n=0$, the ISP should offer the spot transit for free in order to attract demand; when the system is fully utilized, i.e. $n=K=100$, the ISP uses the null price $p^{\max}$ so that no arrival will be observed. $h_n$ is increasing and concave in $n$ as predicted in Theorem~\ref{thm:h_concavity}. Second, we notice that $p^*_n$ decreases for a given $n$ when the departure rate increases, i.e. when the constant $c$ in $\theta(p)=cp^2$ increases. This is intuitive to understand: The ISP has to lower the price when it faces a higher departure rate in order to maintain the customer base. 

On the other hand, as shown in Fig.~\ref{fig:reward123} $h_n/v$ for a given $n$ increases when the departure rate increases, implying that the revenue difference between systems of different initial states diminishes (recall $h_K=0$) with stronger departure dynamics. This is so because with stronger dynamics, it takes shorter time for the system to converge to the steady state and achieve the optimal average revenue in expectation, hence a smaller $|h_n|$. Overall, higher demand dynamics hurts revenue performance despite the effort of dynamic pricing as shown in Table~\ref{table:j}. 

\begin{table}[ht]
\vspace{-2mm}
\caption{Optimal revenue $J^*$ with $K=100$, $\lambda(p)=24-1.5p^2$.}
%\vspace{-2mm}
\small
\centering
\begin{tabular}{|c|c|c|c|c|c|}
    \hline
    $\theta(p)$& $0.3p$ & $0.3p^2$& $0.3p^3$ & $1.5p^2$ & $3p^2$ \\
    \hline
    $J^*$ & 388.7904 & 360.8636 & 304.0449 & 272.7983 & 219.8632  \\
    \hline
  \end{tabular}
\vspace{-2mm}
\label{table:j}
\end{table}

We then consider another class of the function $\theta(p)$ with different exponents. Specifically, we let $\theta(p)=0.3p^c$ with $c=1,2$, and $3$, respectively. This can be considered as varying the price sensitivity of demand departure, with a larger exponent $c$ indicating higher sensitivity. We can see from Fig.~\ref{fig:price514} that when $n$ is small ($<60$), $p^*_n$ slightly increases when the departure rate increases, which contradicts with the observation made above for Fig.~\ref{fig:price123}. The reason is that when $n$ is small $p^*_n$ is less than $1$, and $\theta(p)$ with a larger exponent forces the ISP to adopt a higher price in order to lower the demand departure rate, resulting in the seemingly contradicting but in fact consistent result. The result of $h_n/v$ in Fig.~\ref{fig:reward514} again confirms that higher price sensitivity and stronger dynamics lead to faster convergence to average revenue and smaller revenue differences. The corresponding entries in Table~\ref{table:j} also verify that higher price sensitivity and demand dynamics negatively impact the revenue performance. 

In summary, these results tell us that the demand dynamics has significant impact on ISP's revenue and have to be addressed. Dynamic pricing is important in this regard to mitigate the detrimental effect. The optimal dynamic pricing policy depends on the demand dynamics and is in general increasing with an increase in bandwidth utilization. This can be used to design simple heuristic pricing strategies for large-scale problems with a large number of state variables.



